Sundial: Using Sunlight to Reconstruct Global Timestamps

This paper investigates postmortem timestamp reconstruction in environmental monitoring networks. In the absence of a time-synchronization protocol, these networks use multiple pairs of (local, global) timestamps to retroactively estimate the motes' clock drift and offset and thus reconstruct the measurement time series. We present Sundial, a novel offline algorithm for reconstructing global timestamps that is robust to unreliable global clock sources. Sundial reconstructs timestamps by correlating annual solar patterns with measurements provided by the motes' inexpensive light sensors. The surprising ability to accurately estimate the length of day using light intensity measurements enables Sundial to be robust to arbitrary mote clock restarts. Experimental results, based on multiple environmental network deployments spanning a period of over 2.5 years, show that Sundial achieves accuracy as high as 10 parts per million (ppm), using solar radiation readings recorded at 20 minute intervals.

==> disc.tex <==
\section{Discussion}
\label{sec:disc}

Potentially, one can exploit the correlation in many ways to
reconstruct the timestamp. As an example, one can make use of
the ambient temperature of the motes and the weather stations
nearby to reconstruct the global timestamps. 
A subtle, but important thing to realize is that the motes
local clocks contains a skew. One needs to correct for this 
skew ($\alpha$) before exploiting this correlation. We have 
seen that the skew values can be significantly different for
different deployments (or mote-types). Furthermore, they show 
variation even within a mote-type. Sundial provides a natural
and robust way to extract the skew. Furthermore, the solar model
is very well understood and is not susceptible to effects of
micro-climates. However, we admit that we did not attempt to
recover timestamps using other modalities and we leave this
as a subject of future work.







==> experiments.tex <==
\section{Experiments}
\label{sec:exp}

Consider the following cases : \\
a) We have anchor points and can produce the fit. Use sundial metrics to validate
the reconstruction \\ 
b) We have anchor points but do not know how to associate them 
. i.e. Which segments they belong to (Problem 2, Section ~\ref{sec:prob})
. Use Hough transform to resolve which anchor points are part of the 
same data segment and we can use the sundial to resolve which fits
correspond to which segments. \\
c) We do not have any anchor points at all but the segments of data
are for long contiguous stretches. Use the LOD pattern 
to correlate and work backwards \\
d) We do not have any anchor points but the segments of data are
short and bursty $ \rightarrow $ HOPELESS !


==> graphs/etc.tex <==
% ----- comments ---------


\begin{comment}
%-------------------------------------------------
% Table of nodes and segments
%-------------------------------------------------

\begin{table}
\caption{Nodes, segments and the number of days for each of the segments. The
	two different deployments are indicated using the letter $L$ and $J$
	.} 
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Deployment}  &  \textbf{Node ID}  &  \textbf{Segment number}  & \textbf{Days of Deployment} \\
\hline
$L$ & 71  & 3  & 341  \\  
\hline 
$L$ & 72 & 1 & 587 \\
\hline
$L$ & 73 & 1  & 481  \\  
\hline
$L$ & 74  & 2 &  567 \\  
\hline
$L$ & 75 & 4 & 308  \\  
\hline
$L$ & 76 & 1 & 289 \\  
\hline
$J$ & 2 & 1  & 157  \\  
\hline
$J$ & 5 & 1 & 158 \\  
\hline
$J$ & 6 & 1 & 141 \\  
\hline
$J$ & 8 & 1 & 166 \\  
\hline
$J$ & 11 & 1 & 166 \\  
\hline
$J$ & 12 & 1 & 107 \\  
\hline
$J$ & 13 & 1 & 166 \\  
\hline
$J$ & 14 & 1 & 167 \\  
\hline
$J$ & 15 & 1 &  166 \\  
\hline
$J$ & 29 & 1 & 134 \\  
\hline
$J$ & 43 & 1 & 134 \\  
\hline
$J$ & 44 & 1 & 134 \\  
\hline
$J$ & 45 & 1 & 134 \\  
\hline
\end{tabular}
\label{tab:deploy}
\end{center}
\end{table}

%-------------------------------------------------
% End of table
%-------------------------------------------------


\end{comment}



\begin{comment}


\begin{figure}[t]
	\centering
	\setcounter{subfigure}{0}
	\subfigure[RMS error in days]{
		\label{sfig:dayerr}
                \includegraphics[scale=0.5]{./graphs/error-days.pdf}
	}\,
	\setcounter{subfigure}{1}
	\subfigure[RMS error in minutes]{
		\label{sfig:minerr}
                \includegraphics[scale=0.5]{./graphs/error-minutes.pdf}
	} \\
	\setcounter{subfigure}{2}
	\subfigure[Relationship between $\rho_{max}$ and day-error]{
		\label{sfig:corr-day}
                \includegraphics[scale=0.5]{./graphs/corr-vs-day.pdf}
	}
	\setcounter{subfigure}{3}
	\subfigure[]{
		\label{sfig:alpha}
                \includegraphics[scale=0.5]{./graphs/alpha.pdf}
	} \\
	\caption{}
        \label{fig:sundial-res}
\end{figure}

\end{comment}


\begin{comment}

\subsection{Bad Anchor Points}
\label{subsec:gcproblem}

The veracity of anchor points plays a pivotal role in the
reconstruction of timestamps. Drifting base-stations and inaccurate
clock sources can often corrupt anchor points. Figure \ref{fig:drift}
shows how minor errors in $\alpha$ estimation can lead to huge errors
in reconstruction over time.  It is important to realize that having
accurate anchor points is the key in obtaining accurate estimates for
the $\alpha$ and $\beta$ parameters.  At the same time, failures in
global clocks represent realistic situations and safeguarding the
timestamp reconstruction process to detect bad anchor points is
critical. It is worth mentioning here that often times only a few
anchor points might contain errors. In such situations, censoring
those bad anchor points can provide good reconstruction.  On the other
hand, anchor points obtained from a clock source that has a gradual
drift is more deceptive.  This would result in bad estimates of
$\alpha$, resulting in an inaccurate reconstruction that can
potentially go unnoticed.


\end{comment}


% comment out
\begin{comment}
In this section we provide a detailed account of our robust
methodology to gracefully handle problems described in Section
\ref{sec:prob}. We begin by describing a robust timestamp
reconstruction algorithm that takes as input anchor points for a given
mote. Note that the data could have multiple segments and these anchor
points could belong to any of the data segments. Furthermore, some of
these anchor points could be bad. Our algorithm elegantly addresses
both these issues and produces a robust estimate of $\alpha$ and
$\beta$ parameters for each segment of the mote.
\end{comment}


\begin {comment}

% previous abstract
% jg : I keep it here in case we want to refer to it.

In this paper we explore the problem of postmortem reconstruction of
global timestamps for environmental wireless sensor networks that use
only local clocks for timestamping their recording measurements. First
part of our contribution consists in a robust method of deriving the
global timestamps in the presence of faulty (global timestamps, local
timestamps) pairs. The second part is represented by a novel way of
finding the global timestamps using the information provided by cheap
light sensors. The solution does not rely on any global clock readings
and our results shows that is capable to provide 10-100 ppm accuracy
using a sampling rate of one light reading each 20 minutes.
\end{abstract}

\end{comment}

==> lessons.tex <==
\section{Lessons}
\label{sec:eval}
We can talk about the idea of keeping a journal. This has helped us in
two ways : \\
1) The anchors points are more regular so the fit is better \\
2) The use of the logcookie helps us in associating clock fits to data segments

